Human-Based Risk Model for Improved Driver Support in Interactive Driving Scenarios

This paper addresses the problem of human-based driver support. Nowadays, driver support systems help users to operate safely in many driving situations. Nevertheless, these systems do not fully use the rich information that is available from sensing the human driver. In this paper, we therefore present a human-based risk model that uses driver information for improved driver support. In contrast to state of the art, our proposed risk model combines a) the current driver perception based on driver errors, such as the driver overlooking another vehicle (i.e., notice error), and b) driver personalization, such as the driver being defensive or confident. In extensive simulations of multiple interactive driving scenarios, we show that our novel human-based risk model achieves earlier warning times and reduced warning errors compared to a baseline risk model not using human driver information.

==> chapters/warning.tex <==
\section{Warning System}
\label{sec:warning_system}
In the last section, we described the risk factor and how it can be estimated with Risk Maps. We want to use the risk factor to better warn and support the driver. In this section, we therefore describe how we adapt the driver support based on the risk factor.

\subsection{Adapting Warning Signal}

The warning system consists of two modules. The factor estimation module that estimates the driver type of the user of the system and the warning adapation module that checks the risk for the driver type and warns the driver. The factor estimation module results in a personalized risk plot.

\begin{itemize}
 \item Personalized risk plot shows how the driver perceives the future driving situation. 
 \item The factor changes the size of the risk spot in the risk plot. For example, a small factor would result in a smaller risk spot and a large factor in a larger risk spot.
\end{itemize}

The warning module takes the risk factor changes for a warning into account. We predict constant velocity for the driver and check the personalized risk value for this behavior. In addition, we add the risk factor as a weight onto the risk value to describe the warning signal $W$. We therefore retrieve
\begin{equation}
W(t) = f_{\alpha} * R(\alpha)
\label{eq:warning_signal}
\end{equation}
The risk factor $f_{\alpha}$ is dependent on the personalization $\alpha$. Is linear function going from 0.01 for densive driver over 1.0 for normal driver to 2 for confident driver.
\footnote{Remark: It is not necessary to compute the whole risk plot for the perosnalized risk. One single evaluation of the risk for constant velocity $R_{\text{pers}}$ is sufficient to warn the user. However, for explainability, we compute the whole plot in this paper.}

\begin{itemize}
 \item The personalized risk spot matches the driver and thus the warning signal should align to the driver's feeling of risk.
\end{itemize}
As a comparison, state of the art would only use the risk value resulting from constant velocity predictions or other predictions from the agents without a personalized risk factor or general parametrization of the risk model. 


